Automated Extraction and Analysis of Developer's Rationale in Open Source Software

Contributors to open source software must deeply understand a project's history to make coherent decisions which do not conflict with past reasoning. However, inspecting all related changes to a proposed contribution requires intensive manual effort, and previous research has not yet produced an automated mechanism to expose and analyze these conflicts. In this article, we propose such an automated approach for rationale analyses, based on an instantiation of Kantara, an existing high-level rationale extraction and management architecture. Our implementation leverages pre-trained models and Large Language Models, and includes structure-based mechanisms to detect reasoning conflicts and problems which could cause design erosion in a project over time. We show the feasibility of our extraction and analysis approach using the OOM-Killer module of the Linux Kernel project, and investigate the approach's generalization to five other highly active open source projects. The results confirm that our automated approach can support rationale analyses with reasonable performance, by finding interesting relationships and to detect potential conflicts and reasoning problems. We also show the effectiveness of the automated extraction of decision and rationale sentences and the prospects for generalizing this to other open source projects. This automated approach could therefore be used by open source software developers to proactively address hidden issues and to ensure that new changes do not conflict with past decisions.

==> listings/prompt_chatGPT.tex <==
\definecolor{bg}{rgb}{0.95,0.95,0.95}

\begin{figure}
\centering

\begin{mdframed}[]
\scriptsize

% \begin{minted}[breaklines,frame=single]{python}
\begin{minted}[breaklines]{python}
prompt = """ Which chunks of this sentence indicate Decision and which chunks indicate Rationale? 
 
Decision is an action or a change that has been made, including a description of the patch behaviour.
Rationale is the reason for a decision or value judgment.

Your answer should be strictly in this format: 
Decision: XX
Rationale: YY 
XX and YY must be chunks from the sentence in question. 
All sentences express both a Decision and the Rationale behind it.
If you still can not find the decision or the rationale, only answer "None" instead of XX or YY.
Do not add any other text in your answer.

Example1: 
s = "Remove the mm_kill() function call because we do not use it anymore"
Decision: Remove the mm_kill() function call
Rationale: we do not use it anymore
      
Example2: 
s = "Remove the unused mm_kill() function call"
Decision: Remove the unused mm_kill() function call
Rationale: unused

Example3: 
s = "Fix this bug"
Decision: Fix this bug
Rationale: Fix

Sentence : """
\end{minted}
\end{mdframed}
\caption{The prompt used to interact with ChatGPT \bentley{Might be better to have this online. I think we should focus the paper more on the structuring and the binary classifiers (more mature techniques), rather than the LLM work (less mature)}}\label{fig:prompt_chatGPT}
\end{figure}

==> tables/binary_classification_decision_rationale_supporting_facts.tex <==
\begin{table}[tp]
    \footnotesize
     \caption{Binary classification evaluation (10 fold ) }
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \toprule
      \multirow{2}{*}{\textbf{Model}}  & \multicolumn{4}{c|} {\textbf{Decision}} &  \multicolumn{4}{c|} {\textbf{Rationale}}& 
       \multicolumn{4}{c|} {\textbf{Supporting Facts}}\\
       \cmidrule{2-13}
          & Accuracy & Precision & Recall & F1 & Accuracy & Precision & Recall & F1 & Accuracy & Precision & Recall & F1  \\
        
          \midrule
         
         Logistic Regression & 0.70  & 0.70 & 0.87  & 0.78  
         & 0.68 & 0.69 & 0.80 & 0.74  
         & 0.78  & 0.75 &0.85  & 0.80  \\

          \midrule
          
          Decision Tree & 0.63  & 0.70  & 0.69 & 0.69
          & 0.62 & 0.66 & 0.65 & 0.66
          & 0.69 & 0.71  & 0.70 & 0.71 \\
           \midrule
             
          SVM & 0.70 & 0.70 & 0.87 & 0.78 & 
          0.69  &  0.69  &  0.80 &  0.74& 
          0.77   & 0.74  & 0.88 & 0.80 \\

         \midrule
            
        LSTM &0.90 & 0.92 &0.92 & 0.92 
        & \textbf{0.90}  & 0.91  &\textbf{ 0.91}& \textbf{0.91} & 0.87  &  0.83 & 0.83& 0.83 \\

       \midrule
        Bi-LSTM & \textbf{0.92}& \textbf{0.93} & \textbf{0.94}& \textbf{0.93} 
        &\textbf{ 0.90}& \textbf{0.92}  &0.90 &\textbf{0.91} 
        & \textbf{0.91} & \textbf{0.91}  & \textbf{0.93} & \textbf{0.92} \\
      \midrule

        DistilBERT & 0.81 &  0.82 & 0.87 & 0.84 & 
                     0.73 & 0.75  & 0.77 & 0.76  & 
                 0.84 &  0.85 & 0.83 & 0.84 \\

         \midrule    
        ALBERT (large) & 0.80 & 0.82 & 0.85 & 0.83 & 
                 0.73  & 0.75  & 0.80& 0.77 & 
                0.82 & 0.84  & 0.83 & 0.83 \\
       \midrule
        
        BERT (large) & 0.81 & 0.84 & 0.85 & 0.84 & 
                  0.74 & 0.75  &0.80 & 0.77 & 
                  0.83 & 0.85  & 0.83 & 0.84 \\
       \midrule

        RoBERTa (large) & 0.81 & 0.84 &0.86 &0.84 & 
                 0.75   &  0.76 & 0.82& 0.78 & 
                0.82 & 0.84  & 0.82 & 0.83 \\

        \bottomrule
          
    \end{tabular}
   
    \label{tab:binary_classification}
\end{table}



==> tables/mapping.tex <==

\begin{table}[]
\footnotesize
    \centering
    \begin{tabular}{p{0.3cm}|p{1cm}|p{3.2cm}|p{7.2cm}|p{0.4cm}}
    \toprule
        C. & RQ. & R. sub-Q / Contribution  & Metric (\textbf{m}) / Correctness validation (\textbf{v}) & Sect. \\
    \midrule
    
    1 & \multirow{4}{*}{\makecell{RQ.1 : \\ feasibili- \\ty \\ (using \\ the \\ OOM- \\ Killer \\ module \\ example) }}& RQ.1.1 : ability to find similar and contradictory decisions & 
\textbf{m}: number of similar and contradictory decisions detected. \newline \textbf{v}: manual validation of some entities + relationships (Tables~\ref{tab:chatgpt_limitation_sentences},~\ref{tab:similarities_contradiction_examples}).
& \ref{sec:rationale_structuring}\\
\cmidrule{1-1} \cmidrule{3-5}

     2 &  & 
       RQ.1.2 : ability to detect inconsistencies & 
        
      \textbf{m}: number of inconsistencies detected. \newline
      \textbf{v}: manual  investigation of a sample (Table~\ref{tab:inconsistencies}). & \ref{sec:validation_mechanisms} \\
    \cmidrule{1-1} \cmidrule{3-5}

      
     1,2 & & RQ.1.3 : performance  & \textbf{m}: time needed to create the graph. & \ref{sec:performance} \\
\cmidrule{1-1} \cmidrule{3-5}
       
    3 & &  RQ.1.4 : effectiveness of the automatic extraction of decision and rationale sentences  &  
    \textbf{m}: performance of the best classifiers on the OOM-Killer dataset using standard evaluation metrics (Table~\ref{tab:bi_lstm_performance}) + comparison to the human performance (Table~\ref{tab:raters}). & \ref{sec:rationale_extraction} \\
    \midrule
    \multirow{2}{*}{4} & \makecell{RQ.2 : \\ generali- \\ zability} &   Generalizability of the best classifiers & 
    Other Linux Modules: \textbf{v}:  manual validation of some  predictions + inter-rater agreement (Table~\ref{tab:generalization_linux}).
    \newline Other OSS: \textbf{m}: comparison with the original labelling (Table~\ref{tab:os_generalization_results}).
    & \ref{sec:classification_generalization} \\ 
   \cmidrule{2-5}

     & & Inconsistency detection in other contexts & 
     \textbf{m}: number of inconsistencies detected (Table~\ref{tab:project_statistics}). \newline
      \textbf{v}: manual  investigation of a sample (Table~\ref{tab:inconsistencies_validation}).  & \ref{sec:application}  \\ 

    
         \bottomrule
    \end{tabular}
    \caption{\added{Mapping between RQs and sub-questions, metrics used to answer them, process used to validate correctness of extracted information, components of our methodology and article sections.}}
    \label{tab:my_label}
\end{table}

==> tables/raters_decision_rationale_supportin_facts.tex <==
\begin{table}[tp]
    \footnotesize
     \caption{Human performance \mouna{maybe just keep accuracy here ? all these values are over-kill}}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \toprule
      \multirow{2}{*}{\textbf{Rater}}  & \multicolumn{4}{c|} {\textbf{Decision}} &  \multicolumn{4}{c|} {\textbf{Rationale}}& 
       \multicolumn{4}{c|} {\textbf{Supporting Facts}}\\
       \cmidrule{2-13}
          & Accuracy & Precision & Recall & F1 & Accuracy & Precision & Recall & F1 & Accuracy & Precision & Recall & F1  \\
        
         \midrule
         
        R1 &0.94 & \textbf{1.0} & \textbf{0.91} & \textbf{0.95}& 
                 0.83  & 1.0  &0.69 & 0.82 & 
              0.80   & 1.0  & 0.62 & 0.77 \\

         \midrule    
        R2 & \textbf{0.95} & \textbf{1.0} & \textbf{0.91} & \textbf{0.95} & 
                \textbf{0.86}   & \textbf{1.0}  & 0.75& 0.85 & 
                0.87 & 1.0  & 0.76 & 0.86 \\
       \midrule
        
        R3 & 0.83& 1.0 & 0.73&0.84 & 
        \textbf{0.86}  & \textbf{1.0}  &\textbf{0.76} &\textbf{0.86}  & 
              \textbf{0.95}   & \textbf{1.0}  & \textbf{0.90}  & \textbf{0.95}  \\

        \bottomrule
          
    \end{tabular}
   
    \label{tab:raters}
\end{table}

==> text/viz.tex <==
\subsubsection{Visualization}
To visualize the graph, we use 
Neo4j graph database~\cite{miller2013graph}.
Figure~\ref{fig:neo4j} shows an excerpt from the Decision and Rationale graph. We argue that the visualization helps comprehension. Our future work includes a user study that will evaluate this claim about the usefulness of the visualization.  
% \todo{Can I get the whole graph as SVG  ? and put it in the replication package? TODO: write another code for that ? or maybe just put the fig for 500-600 in the package}

%%%% To get the figure:
% 1.download SVG from NEO4J (the whole graph)
% 2. open it with Insckape and Clip the part that I want (create regtangle shape, go back to selection mode, zoom out, shift + select whole figure also,  set clip) https://youtu.be/wIx9U2HQbJA?t=221 
% 3. export that part/selection (panel at right) as png picture 
% Note: including SVG causes error
%%%%%%
 \begin{figure}[tbh]
    \centering
    \frame{\includegraphics[width = 0.4\textwidth]{./figs/g1840.png}}
    \caption{An excerpt from the Decision and Rationale graph.}
    % the graph is obtained with running df[500-600 ]
    \label{fig:neo4j}
\end{figure}
